Byzantine Distributed Function Computation

We study the distributed function computation problem with $k$ users of which at most $s$ may be controlled by an adversary and characterize the set of functions of the sources the decoder can reconstruct robustly in the following sense -- if the users behave honestly, the function is recovered with high probability (w.h.p.); if they behave adversarially, w.h.p, either one of the adversarial users will be identified or the function is recovered with vanishingly small distortion.

==> figures.tex <==
\iffalse
\newcommand{\height}{0.5}
\newcommand{\width}{0.5}

\newcommand \drawbox[1]
{
    \draw[draw=black] (0,0) rectangle ++(0.7,0.4);
}

\begin{figure}
    \begin{center}
        \begin{tikzpicture}
            \drawbox{0}
        \end{tikzpicture}
    \end{center}
\end{figure}
\fi

==> neha.tex <==
\section{Neha}

\iffalse
\begin{proof}[Proof of Lemma~\ref{lem:2user-typicality}]
Part (i) of the lemma follows from standard properties of types [\cite, ~\ref{}]. We show part (ii) now.






From Lemma~\ref{lem:2user-technical-single-letter}, we obtain a function $\gamma': \mathbb{R}^{+} \rightarrow \mathbb{R}^{+}$ such that $\gamma'(\delta) \rightarrow 0$ as $\delta \downarrow 0$ satisfying the following: if $W_{\bX_1|X_1}$ is such that the p.m.f. $Q_{\uX_1 \uX_2 \uY}(\ux_1,\ux_2,\uy):= \sum_{x_1} P_{X_1 X_2 Y}(x_1, x_2, y) W_{\bX_1|X_1}(\ux_1|x_1)$ belongs to $\cV_1^{\delta} \cap \cV_2^{\delta}$, then, 
\begin{equation}\label{eq:2user-typicality-1}
    \pr(f(X_1,X_2,Y) \neq g(\bX_1,X_2,Y)) \leq \gamma'(\delta)
\end{equation}
under the p.m.f. $P_{X_1 X_2 Y} W_{\bX_1|X_1}$. This implies that 
\begin{align*}
\sum_{x_1, x_2, y, \ux_1}P_{X_1 X_2 Y}(x_1, x_2, y) W_{\bX_1|X_1}(\ux_1|x_1)\mathbb{1}_{f(x_1,x_2,y) \neq g(\bx_1,x_2,y)} \leq \gamma'(\delta)
\end{align*} or for any $(x_1^n, x_2^n, y^n, \ux_1^n)$ with joint empirical type $P_{X_1 X_2 Y}(x_1, x_2, y) W_{\bX_1|X_1}(\ux_1|x_1)$, we have
\begin{align*}
\ham(f(x_1^n,x_2^n,y^n), g(\bx_1^n,x_2^n,y^n))\leq \gamma'(\delta).
\end{align*}


We denote the probability that we are interested in bounding by $\cE'(n,\gamma)$, i.e., we have, 
\begin{multline*}
\cE'(n,\gamma) = \pr\left((\type{\bX_1^n X_2^n Y^n} \in \cV_1^{\delta} \cap \cV_2^{\delta}) \cap \right.\\ \left.(\ham(f(X_1^n,X_2^n,Y^n),g(\bX_1^n,X_2^n,Y^n))>\gamma(\delta))\right),
\end{multline*}
\red{*******************}

Define $\gamma(\delta) = \frac{\gamma'(2\delta)}{p_{\text{min}}}$ where $p_{\text{min}} = \min_{(a,b,c): P_{X_1 X_2 Y}(a,b,c)>0}P_{X_1 X_2 Y}(a,b,c)$. 





We denote the probability that we are interested in bounding by $\cE'(n,\gamma)$, i.e., we have, 
\begin{multline*}
\cE'(n,\gamma) = \pr\left((\type{\bX_1^n X_2^n Y^n} \in \cV_1^{\delta} \cap \cV_2^{\delta}) \cap \right.\\ \left.(\ham(f(X_1^n,X_2^n,Y^n),g(\bX_1^n,X_2^n,Y^n))>\gamma(\delta))\right),
\end{multline*}
which can be rewritten as 
\begin{multline*}
    \sum_{x_1^n, x_2^n, y^n} P^n_{X_1 X_2 Y}(x_1^n,x_2^n,y^n) \sum_{\bx_1^n} W_1(\bx_1^n|x_2^n)\\
    \mathbb{1}\left\{\type{\bx_1^n x_2^n y^n} \in \cV_1^{\delta} \cap \cV_2^{\delta},d> \gamma(\delta) \right\},
\end{multline*}
where $d := \ham(f(x_1^n,x_2^n,y^n), g(\bx_1^n,x_2^n,y^n))$.
Let $\varPi_n$ be the set of all permutations over $[n]$. Define $\pi(x^n):= \left(x_{\pi(1)}, \dots, x_{\pi(n)}\right)$ where $\pi \in \varPi_n$. Noting that (i) $(x_1^n,x_2^n,y^n)$ is generated i.i.d. from $P_{X_1 X_2 Y}$, and therefore $P^n_{XYZ}(x_1^n,x_2^n,y^n)$ is invariant under permutations of $(x_1^n,x_2^n,y^n)$ and (ii) $d$ and $\type{\bx_1^n x_2^n y^n}$ are invariant under the permutations of $(x_1^n,x_2^n,y^n)$, we can rewrite $\cE(n,\gamma)$ as
\begin{align*}
    &\frac{1}{\varPi} \sum_{\pi \in \varPi_n} \sum_{x_1^n x_2^n y^n} P^n_{X_1X_2Y}(\pi(x_1^n),\pi(x_2^n),\pi(y^n)) \sum_{\bx_1^n} W_1(\pi(\bx_1^n)|\pi(x_1^n))\\
    &{}\times \mathbb{1}\left\{ \type{\bx_1^n x_2^n y^n} \in \cV_1^{\delta} \cap \cV_2^{\delta},d> \gamma(\delta) \right\}\\
    &=\sum_{x_1^n x_2^n y^n} P^n_{X_1 X_2 Y}(x_1^n,x_2^n,y^n) \frac{1}{\varPi}\sum_{\pi \in \varPi_n}\sum_{\bx_1^n}W_1(\pi(\bx_1^n)|\pi(x_1^n))\\
    &\phantom{==}\times \mathbb{1}\left\{ \type{\bx_1^n x_2^n y^n} \in \cV_1^{\delta} \cap \cV_2^{\delta},d> \gamma(\delta) \right\}\\
    &=\sum_{x_1^n x_2^n y^n} P^n_{X_1 X_2 Y}(x_1^n, x_2^n, y^n) \sum_{\bx_1^n} \Wsym(\bx_1^n|x_1^n)\\
    &\phantom{==}\times \mathbb{1}\left\{\type{\bx_1^n x_2^n y^n} \in \cV_1^{\delta} \cap \cV_2^{\delta}, d>\gamma(\delta)\right\},
\end{align*}
where $\Wsym(\bx_1^n|x_1^n) = \frac{1}{\varPi}\sum_{\pi \in \varPi_n} W_1(\pi(\bx_1^n)|\pi(x_1^n))$.
Decomposing $\cX_1^n$ as the union of type sets obtained by passing $\bx_1^n$ through channels in $\cW(\cX_1|P_{X'_1})$, $\cE'(n,\gamma)$ can be upper bounded by
\begin{align*}
    &\sum_{P_{X_1' X_2' Y'} \in \cP_n(\cX_1 \times \cX_2 \times \cY)} \sum_{(x_1^n,x^n_2,y^n) \in \cT^n_{X_1' X_2' Y'}} P^n_{X_1 X_2 Y}(x_1^n,x_2^n,y^n)\\
    &\phantom{==}\times \sum_{{\bW} \in \cW(\cX_1|P_{X'_1})} \sum_{\bx_1^n \in \cT^n_{\bW}(x_1^n)} \Wsym(\bx_1^n|x^n)\\
    &\phantom{==} \times \mathbb{1}\left\{ \type{\bx_1^n x_2^n y^n} \in \cV_1^{\delta} \cap \cV_2^{\delta}, d> \gamma(\delta) \right\}.
\end{align*}

We now define a set of channels whose view distributions are in $\cV_1^{\delta} \cap \cV_2^{\delta}$,
\begin{multline*}
\cW(\delta) = \left\{\tW_{\bX_1|X_1} \in \cP(\cX_1|\cX_1): \right.\\
\left. \sum_{x_1}P_{X_1 X_2 Y}(x_1,\ux_2,\uy) \tW_{\bX_1|X_1}(\ux_1|x_1) \in \cV_1^{\delta} \cap \cV_2^{\delta} \right\}.
\end{multline*}
Clearly, for any conditional type $\bW \in \cW(2\delta) \cap \cW(\cX_1|P_{X_1'})$, $\pr(f(X_1,X_2,Y)\neq g(\bX_1,X_2,Y)) \leq \gamma'(2\delta)$ under the distribution $P_{X_1 X_2 Y} \bW$, which further implies that for all $(a,b,c): P_{X_1 X_2 Y}(a,b,c)>0$, 
$$\sum_{d \in \cX_1} \bW(d|a) \mathbb{1} \left\{ f(a,b,c) \neq g(d,b,c) \right\} \leq \gamma(\delta).$$
It follows that for a sequence $(x_1^n,x_2^n,y^n)$ and $\bx_1^n \in \cT^n_{\bW}(x^n)$, 
\begin{align*}
    &\ham(f(x_1^n,x_2^n,y^n), g(\bx_1^n,x_2^n,y^n))\\
    &=\sum_{a,d \in \cX_1, b\in \cX_2, c \in \cY} \type{x_1^n x_2^n y^n} (a,b,c) \bW(d|a) \\
    &\phantom{==}\mathbb{1} \left\{ f(a,b,c) \neq g(d,b,c) \right\} \leq \gamma(\delta).
\end{align*}
Using this, along with the fact that
\begin{multline*}
    \Wsym(\bx_1^n|x_1^n) = \frac{\Wsym(\cT^n_{\bW}(x_1^n)|x_1^n)}{|\cT^n_{\bW}(x_1^n)|} \leq \frac{1}{|\cT^n_{\bW}(x_1^n)|}\\ \leq (n+1)^{|\cX_1|^2} \bW(\bx_1^n|x_1^n),
\end{multline*}
(the first equality is due to the fact that since $\Wsym$ is a symmetrized channel, the probability of occurrence of any sequence of type $\cT^n_{\bW}(x_1^n)$ under the channel $\Wsym$ with input $x_1^n$ is the same)

we can upper bound $\cE'(n,\gamma)$ by 
\begin{align*}
    &(n+1)^{|\cX_1|^2} \sum_{P_{X_1' X_2' Y'} \in \cP_n(\cX_1 \times \cX_2 \times \cY)} \sum_{(x_1^n,x^n_2,y^n) \in \cT^n_{X_1' X_2' Y'}}\\
    &P^n_{X_1 X_2 Y}(x_1^n,x_2^n,y^n)
    \sum_{{\bW} \in \cW(\cX_1|P_{X'_1}) \cap \cW(2\delta)^c} \sum_{\bx_1^n \in \cT^n_{\bW}(x_1^n)} \bW(\bx_1^n|x^n)\\
    &\phantom{==} \times \mathbb{1}\left\{ \type{\bx_1^n x_2^n y^n} \in \cV_1^{\delta} \cap \cV_2^{\delta} \right\}\\
    \leq 
    &(n+1)^{|\cX_1|^2} \sum_{P_{X_1' X_2' Y'} \in \cP_n(\cX_1 \times \cX_2 \times \cY)} \sum_{(x_1^n,x^n_2,y^n) \in \cT^n_{X_1' X_2' Y'}}\\
    &P^n_{X_1 X_2 Y}(x_1^n,x_2^n,y^n)
    \sum_{{\bW} \in \cW(\cX_1|\cX_1) \cap \cW(2\delta)^c} \sum_{\bx_1^n \in \cT^n_{\bW}(x_1^n)} \bW(\bx_1^n|x^n)\\
    &\phantom{==} \times \mathbb{1}\left\{ \type{\bx_1^n x_2^n y^n} \in \cV_1^{\delta} \cap \cV_2^{\delta}\right\}\\
    \leq
    &(n+1)^{2|\cX_1|^2} \sup_{\bW \in \cW(\cX_1|\cX_1) \cap \cW(2\delta)^c} 
    \sum_{x_1^n x_2^n y^n} P^n_{X_1 X_2 Y}(x_1^n,x_2^n,y^n)\\
    &\sum_{\bx_1^n} \bW(\bx_1^n|x^n) \mathbb{1}\left\{ \type{\bx_1^n x_2^n y^n} \in \cV_1^{\delta} \cap \cV_2^{\delta}\right\}.
\end{align*}
If $\cP(2\delta) = \left\{ \sum_{a \in \cX} P_{X_1 X_2 Y}(a,b,c) \bW (d|a): \bW \in \cW(\cX_1|\cX_1) \cap \cW(2\delta)^c \right\}$, then, $\cP(2 \delta) \subseteq (\cV_1^{2\delta} \cap \cV_2^{2\delta})$. Using this, we bound $\cE'(n,\gamma)$ with 
$$\sup_{Q_{\bX_1 X_2 Y} \in (\cV_1^{2\delta} \cap \cV_2^{2\delta})^c} \sum_{(\bx_1^nx_2^ny^n)} Q^n_{\bX_1 X_2 Y}(\bx_1^n x_2^n y^n) \mathbb{1} \left\{ \type{\bx_1^n x_2^n z^n} \in \cV_1^{\delta} \cap \cV_2^{\delta} \right\},$$
which is upper bounded by $2^{-\Omega(n)}$ due to ~\ref{lem:typicalityerror}.
\end{proof}
\fi








\iffalse



which can be rewritten as 
\begin{align*}
    &\sum_{x_1^n, x_2^n, y^n} P^n_{X_1 X_2 Y}(x_1^n,x_2^n,y^n) \sum_{\bx_1^n} W_1(\bx_1^n|x_1^n)\\
    &\qquad \qquad \mathbb{1}\left\{\type{\bx_1^n x_2^n y^n} \in \cV_1^{\delta} \cap \cV_2^{\delta},d> \gamma(\delta) \right\}\\
    % & \leq \sum_{\substack{Q_{X_1X_2Y\bX_1}\in \cP_n\inp{\cX_1\times\cX_2\times\cY\times\cX_1}\\ :{Q_{\bX_1X_2Y}}\in \cV_1^{\delta} \cap \cV_2^{\delta}}}\sum_{\substack{(x_1^n, x_2^n, y^n, \bx_1^n)\\\in \cT^n_{X_1X_2Y\bX_1}}}P^n_{X_1 X_2 Y}(x_1^n,x_2^n,y^n)\\
    % &\qquad W_1(\bx^n_1|x^n_2)\mathbb{1}\left\{d> \gamma(\delta) \right\}\\
    & \stackrel{=}{(a)} \sum_{\pi\in \Pi_n}\frac{1}{|\Pi_n|}\sum_{x_1^n, x_2^n, y^n} P^n_{X_1 X_2 Y}(\pi\inp{x_1^n},\pi\inp{x_2^n},\pi\inp{y^n})  \\
    &\qquad \sum_{\bx_1^n}W_1(\pi\inp{\bx_1^n}|\pi\inp{x_1^n})\\
    &\qquad \mathbb{1}\left\{\type{\pi\inp{\bx_1^n} \pi\inp{x_2^n} \pi\inp{y^n}} \in \cV_1^{\delta} \cap \cV_2^{\delta},d> \gamma(\delta) \right\}\\
    & \stackrel{(a)}{=} \sum_{\substack{x_1^n, \\x_2^n, y^n}} P^n_{X_1 X_2 Y}({x_1^n},{x_2^n},{y^n}) \sum_{\bx_1^n} {\sum_{\pi}\frac{1}{|\Pi_n|}W_1(\pi\inp{\bx_1^n}|\pi\inp{x_2^n})}\\
    &\qquad \mathbb{1}\left\{\type{{\bx_1^n} {x_2^n} {y^n}} \in \cV_1^{\delta} \cap \cV_2^{\delta},\red{d> \gamma(\delta)} \right\}\\
        & \stackrel{(b)}{=} \sum_{x_1^n, x_2^n, y^n} P^n_{X_1 X_2 Y}({x_1^n},{x_2^n},{y^n}) \sum_{\bx_1^n} W_{\textsf{sym}}({\bx_1^n}|{x_1^n})\\
    &\qquad \mathbb{1}\left\{\type{{\bx_1^n} {x_2^n} {y^n}} \in \cV_1^{\delta} \cap \cV_2^{\delta},d> \gamma(\delta) \right\}\\
\end{align*}
where $d := \ham(f(x_1^n,x_2^n,y^n), g(\bx_1^n,x_2^n,y^n))$ and $(a)$ follows by noting that $P^n_{X_1 X_2 Y}$ and $d$ are invariant under permutations and in $(b)$, we define $W_{\textsf{sym}}({\bx_1^n}|{x_2^n}) := \inp{\sum_{\pi\in \Pi_n}\frac{1}{|\Pi_n|}W_1(\pi\inp{\bx_1^n}|\pi\inp{x_1^n})}$.

Let \red{ $\cQ_n\inp{\delta}\subseteq \cP_n\inp{\cX_1\times\cX_2\times\cY\times\cX_1}$} be the set of joint types such that for all  $Q_{X_1X_2Y\bX_1}\in \cP_n\inp{\delta}$, we have $D(Q_{X_1X_2Y}||P_{X_1X_2Y})\leq \delta/2$ and $I(X_2Y;\bX_1|X_1)\leq \delta/2$. Then,
\begin{align*}
    &\sum_{x_1^n, x_2^n, y^n} P^n_{X_1 X_2 Y}({x_1^n},{x_2^n},{y^n}) \sum_{\bx_1^n} W_{\textsf{sym}}({\bx_1^n}|{x_1^n})\\
    &\qquad \mathbb{1}\left\{\type{{\bx_1^n} {x_2^n} {y^n}} \in \cV_1^{\delta} \cap \cV_2^{\delta},d> \gamma(\delta) \right\}\\
    & \leq \sum_{\substack{Q_{X_1X_2Y\bX_1}\in \cP_n\inp{\delta}:\\{Q_{\bX_1X_2Y}}\in \cV_1^{\delta} \cap \cV_2^{\delta}}}\sum_{\substack{(x_1^n, x_2^n, y^n, \bx_1^n)\\\in \cT^n_{X_1X_2Y\bX_1}}}P^n_{X_1 X_2 Y}(x_1^n,x_2^n,y^n)\\
    &\qquad \qquad W_{\textsf{sym}}(\bx^n_1|x^n_1)\mathbb{1}\left\{d> \gamma(\delta) \right\}\\
    &\qquad + \sum_{\substack{Q_{X_1X_2Y} \in \cP_n\inp{\cX_1\times\cX_2\times\cY}\\D(Q_{X_1X_2Y}||P_{X_1X_2Y})> \delta/2}}\sum_{\substack{(x_1^n, x_2^n, y^n)\\\in \cT^n_{X_1X_2Y}}}P^n_{X_1 X_2 Y}(x_1^n,x_2^n,y^n)\\
    &\qquad + \sum_{\substack{Q_{X_1X_2Y\bX_1} \\\in \cP_n\inp{\cX_1\times\cX_2\times\cY\times \cX_1}\\I(X_2Y;\bX_1|X_1)> \delta/2}}\sum_{\substack{(x_1^n, x_2^n, y^n)\\\in \cT^n_{X_1X_2Y}}}P^n_{X_1 X_2 Y}(x_1^n,x_2^n,y^n)\\
    &\qquad \qquad \qquad \sum_{\bx_1^n\in \cT^n_{\bX_1|X_1X_2Y}}W_{\textsf{sym}}(\bx^n_1|x^n_1)\\
    & = A+ B + C
\end{align*}
where $d := \ham(f(x_1^n,x_2^n,y^n), g(\bx_1^n,x_2^n,y^n))$. We first analyse $B$.
\begin{align*}
&\sum_{\substack{Q_{X_1X_2Y} \in \cP_n\inp{\cX_1\times\cX_2\times\cY}\\D(Q_{X_1X_2Y}||P_{X_1X_2Y})> \delta/2}}\sum_{\substack{(x_1^n, x_2^n, y^n)\\\in \cT^n_{X_1X_2Y}}}P^n_{X_1 X_2 Y}(x_1^n,x_2^n,y^n)\\
&\stackrel{(a)}{\leq} \sum_{\substack{Q_{X_1X_2Y} \in \cP_n\inp{\cX_1\times\cX_2\times\cY}\\D(Q_{X_1X_2Y}||P_{X_1X_2Y})> \delta/2}}\exp{-nD(Q_{X_1X_2Y}||P_{X_1X_2Y}}\\
&\stackrel{(b)}{\leq} (n+1)^{|\cX_1||\cX_2||\cY|}\exp\inp{-n\delta/2}\\
&\rightarrow 0 
\end{align*} where $(a)$ follows from \eqref{eq:type1} and $(b)$ follows from \eqref{eq:type4}. Now, we analyse $C$.
\begin{align*}
&\sum_{\substack{Q_{X_1X_2Y\bX_1} \\\in \cP_n\inp{\cX_1\times\cX_2\times\cY\times \cX_1}\\I(X_2Y;\bX_1|X_1)> \delta/2}}\sum_{\substack{(x_1^n, x_2^n, y^n)\\\in \cT^n_{X_1X_2Y}}}P^n_{X_1 X_2 Y}(x_1^n,x_2^n,y^n)\\
    &\qquad \qquad \qquad \sum_{\bx_1^n\in \cT^n_{\bX_1|X_1X_2Y}(x_1^n, x_2^n, y^n)}W_{\textsf{sym}}(\bx^n_1|x^n_1)\\
&\stackrel{(a)}{\leq}    \sum_{\substack{Q_{X_1X_2Y\bX_1} \\\in \cP_n\inp{\cX_1\times\cX_2\times\cY\times \cX_1}\\I(X_2Y;\bX_1|X_1)> \delta/2}}\sum_{\substack{(x_1^n, x_2^n, y^n)\\\in \cT^n_{X_1X_2Y}}}P^n_{X_1 X_2 Y}(x_1^n,x_2^n,y^n)\\
    &\qquad \qquad \exp\inp{nH(\bX_1|X_1X_2Y)} (n+1)^{|\cX_1|^2}\exp\inp{-H(\bX_1|X_1}\\
    &\stackrel{(b)}{\leq}\sum_{\substack{Q_{X_1X_2Y\bX_1} \\\in \cP_n\inp{\cX_1\times\cX_2\times\cY\times \cX_1}\\I(X_2Y;\bX_1|X_1)> \delta/2}}(n+1)^{|\cX_1|^2}\exp\inp{-n\delta/2}\\
    &\leq (n+1)^{|\cX_1||\cX_2||\cY||\cX_1}(n+1)^{|\cX_1|^2}\exp\inp{-n\delta/2}\\
    & \rightarrow 0.
\end{align*} where $(a)$ follows by noting that $W_{\textsf{sym}}(\bx^n_1|x^n_1)$ is the same for all $\bx^n_1\in \cT^n_{\bX_1|X_1}(x^n_1)$ and hence by using, $\sum_{\bx^n_1\in \cT^n_{\bX_1|X_1}(x^n_1)}W_{\textsf{sym}}(\bx^n_1|x^n_1)\leq 1$, we have  $W_{\textsf{sym}}(\bx^n_1|x^n_1)\leq \frac{1}{|\cT^n_{\bX_1|X_1}(x^n_1)|}\leq (n+1)^{|\cX_1|^2}\exp\inp{-H(\bX_1|X_1)}$ from \eqref{eq:type3}\red{use $X_1'$ for types. see 5 page}. The inequality $(b)$ follows from  $H(\bX_1|X_1) - H(\bX_1|X_1X_2Y) = I(\bX_1;X_2Y|X_1)> \delta/2$.

Next, we show that $A =0$. \red{write its analysis first}

This will be a consequence of the following corollary to Lemma~\ref{lem:2user-technical-single-letter}. 
\begin{corollary}\label{corollary: 17}
For a 1-viable $f$ along with $g$ as in Lemma~\ref{lem:decoding-function-2user}, parameters $\delta, \beta>0$, there is a $\gamma''(\delta, \beta)$ such that $\lim_{\delta, \beta\to 0} \gamma''(\delta, \beta)=0$
%$\gamma'(\delta)\to 0$ as $\delta\to 0$ 
satisfying the following: if 
$Q_{X_1X_2Y\bX_1}$ is such that $Q_{\bX_1X_2Y}$ belongs to $\cV_1^{\delta}\cap\cV_2^{\delta}$ and there is a $W$ for which $\dtv(Q_{X_1X_2Y\bX_1},P_{X_1X_2Y}W)\leq \beta$, then $\pr(f(X_1,X_2,Y)\neq g(\bX_1,X_2,Y))\leq \gamma''(\beta, \delta)$ under the p.m.f. $Q_{X_1X_2Y\bX_1}$. 
% Suppose $Q_{X_1X_2Y\bX_1}$ is such that there exists a $\bar{W}:\cX_1\rightarrow \cX_1$ satisfying $d_{TV}(Q_{X_1X_2Y\bX_1},P_{X_1X_2Y}W_{1})\leq \beta$ and $Q_{\bX_1X_2Y}\in \cV_1^{\delta} \cap \cV_2^{\delta}$. Then, there exists $\gamma''(\beta, \delta)$ where $\gamma''(\beta, \delta)\rightarrow 0$ as $\beta, \delta\rightarrow 0$ such that $\bbP\inp{f(X_1, X_2, Y)\neq g(\bX_1, X_2, Y)}\leq \gamma''(\beta, \delta)$ under the distribution $Q_{X_1X_2Y\bX_1}$.
\end{corollary}

% \begin{corollary}\label{corollary: 17}
% Suppose $Q_{X_1X_2Y\bX_1}$ is such that there exists a $\bar{W}:\cX_1\rightarrow \cX_1$ satisfying $d_{TV}(Q_{X_1X_2Y\bX_1},P_{X_1X_2Y}W_{1})\leq \beta$ and $Q_{\bX_1X_2Y}\in \cV_1^{\delta} \cap \cV_2^{\delta}$. Then, there exists $\gamma''(\beta, \delta)$ where $\gamma''(\beta, \delta)\rightarrow 0$ as $\beta, \delta\rightarrow 0$ such that $\bbP\inp{f(X_1, X_2, Y)\neq g(\bX_1, X_2, Y)}\leq \gamma''(\beta, \delta)$ under the distribution $Q_{X_1X_2Y\bX_1}$.
% \end{corollary}

For any joint type $Q_{X_1X_2Y\bX_1}\in \cP_n\inp{\delta}$, we have $D(Q_{X_1X_2Y\bX_1}||P_{X_1X_2Y}Q_{\bX_1|X_1})\leq \delta$ and hence $d_{TV}(Q_{X_1X_2Y\bX_1},P_{X_1X_2Y}Q_{\bX_1|X_1})\leq \sqrt{\frac{\delta}{2}}$ (using Pinsker's inequality). Setting $\beta = \sqrt{\delta/2}$, we conclude from Corollary~\ref{corollary: 17} that 
\begin{align*}
\gamma''&(\beta, \delta)\geq \bbP\inp{f(X_1, X_2, Y)\neq g(\bX_1, X_2, Y)}\\
&\sum_{x_1,  x_2, y, \bx_1}Q_{X_1X_2Y\bX_1}(x_1, x_2, y, \bx_1)\mathbb{1}_{\inp{f(x_1, x_2, y)\neq g(\bx_1, x_2, y)}}.
\end{align*}
For $\gamma(\delta):=\gamma''(\sqrt{\delta/2}, \delta)$, we conclude that for all sequences $(x_1^n, x_2^n, y^n, \bx_1^n)$ of joint type $Q_{X_1X_2Y\bX_1}$, we have $\ham(f(X_1^n,X_2^n,Y^n),g(\bX_1^n,X_2^n,Y^n)\leq \gamma(\delta)$. Hence, $A = 0$.




\subsubsection{Proof of DMC case (will be removed from here)}

 We denote the probability that we are interested in bounding by $\cE'(n,\gamma)$, i.e., we have, 
\begin{multline*}
\cE'(n,\gamma) = \pr\left((\type{\bX_1^n X_2^n Y^n} \in \cV_1^{\delta} \cap \cV_2^{\delta}) \cap \right.\\ \left.(\ham(f(X_1^n,X_2^n,Y^n),g(\bX_1^n,X_2^n,Y^n))>\gamma(\delta))\right),
\end{multline*}
% Note that for any $(x_1^n, x_2^n, y^n, \bar{x}_1^n)\in \cT_{X_1, X_2, Y, \bar{X}_1}$, if $\ham(f(x_1^n,x_2^n,y^n),g(\bx_1^n,x_2^n,x^n))>\gamma(\delta)$. Then, 

Let $\cP_n\inp{\delta}\subseteq \cP_n\inp{\cX_1\times\cX_2\times\cY\times\cX_1}$ be the set of joint types such that for all  $Q_{X_1X_2Y\bX_1}\in \cP_n\inp{\delta}$, we have $D(Q_{X_1X_2Y\bX_1}||P_{X_1X_2Y}W_{1})\leq \delta$. 
\begin{align*}
    &\sum_{x_1^n, x_2^n, y^n, \bx_1^n} P^n_{X_1 X_2 Y}(x_1^n,x_2^n,y^n) W^n_1(\bx^n_1|x^n_2)\\
    &\qquad\mathbb{1}\left\{\type{\bx_1^n x_2^n y^n} \in \cV_1^{\delta} \cap \cV_2^{\delta},d> \gamma(\delta) \right\}\\
    & \leq \sum_{\substack{Q_{X_1X_2Y\bX_1}\in \cP_n\inp{\delta}:\\{Q_{\bX_1X_2Y}}\in \cV_1^{\delta} \cap \cV_2^{\delta}}}\sum_{\substack{(x_1^n, x_2^n, y^n, \bx_1^n)\\\in \cT^n_{X_1X_2Y\bX_1}}}P^n_{X_1 X_2 Y}(x_1^n,x_2^n,y^n)\\
    &\qquad W^n_1(\bx^n_1|x^n_2)\mathbb{1}\left\{d> \gamma(\delta) \right\}\\
    &\qquad + \sum_{Q_{X_1X_2Y\bX_1}\in \cP_m\inp{\delta}^c}\sum_{\substack{(x_1^n, x_2^n, y^n, \bx_1^n)\\\in \cT^n_{X_1X_2Y\bX_1}}}P^n_{X_1 X_2 Y}(x_1^n,x_2^n,y^n)\\
    &\qquad W^n_1(\bx^n_1|x^n_2)\\
    & = A+ B
\end{align*}
where $d := \ham(f(x_1^n,x_2^n,y^n), g(\bx_1^n,x_2^n,y^n))$.

We now need to argue that $A$ and $B$ are small. We will next show that $A=0$. This will be a consequence of the following corollary to Lemma~\ref{lem:2user-technical-single-letter}. 
\begin{corollary}\label{corollary: 17}
For a 1-viable $f$ along with $g$ as in Lemma~\ref{lem:decoding-function-2user}, parameters $\delta, \beta>0$, there is a $\gamma''(\delta, \beta)$ such that $\lim_{\delta, \beta\to 0} \gamma''(\delta, \beta)=0$
%$\gamma'(\delta)\to 0$ as $\delta\to 0$ 
satisfying the following: if 
$Q_{X_1X_2Y\bX_1}$ is such that $Q_{\bX_1X_2Y}$ belongs to $\cV_1^{\delta}\cap\cV_2^{\delta}$ and there is a $W$ for which $\dtv(Q_{X_1X_2Y\bX_1},P_{X_1X_2Y}W)\leq \beta$, then $\pr(f(X_1,X_2,Y)\neq g(\bX_1,X_2,Y))\leq \gamma''(\beta, \delta)$ under the p.m.f. $Q_{X_1X_2Y\bX_1}$. 
% Suppose $Q_{X_1X_2Y\bX_1}$ is such that there exists a $W_1:\cX_1\rightarrow \cX_1$ satisfying $d_{TV}(Q_{X_1X_2Y\bX_1},P_{X_1X_2Y}W_{1})\leq \beta$ and $Q_{\bX_1X_2Y}\in \cV_1^{\delta} \cap \cV_2^{\delta}$. Then, there exists $\gamma''(\beta, \delta)$ where $\gamma''(\beta, \delta)\rightarrow 0$ as $\beta, \delta\rightarrow 0$ such that $\bbP\inp{f(X_1, X_2, Y)\neq g(\bX_1, X_2, Y)}\leq \gamma''(\beta, \delta)$ under the distribution $Q_{X_1X_2Y\bX_1}$.
\end{corollary}

% \begin{corollary}\label{corollary: 17}
% Suppose $Q_{X_1X_2Y\bX_1}$ is such that there exists a $W_1:\cX_1\rightarrow \cX_1$ satisfying $d_{TV}(Q_{X_1X_2Y\bX_1},P_{X_1X_2Y}W_{1})\leq \beta$ and $Q_{\bX_1X_2Y}\in \cV_1^{\delta} \cap \cV_2^{\delta}$. Then, there exists $\gamma''(\beta, \delta)$ where $\gamma''(\beta, \delta)\rightarrow 0$ as $\beta, \delta\rightarrow 0$ such that $\bbP\inp{f(X_1, X_2, Y)\neq g(\bX_1, X_2, Y)}\leq \gamma''(\beta, \delta)$ under the distribution $Q_{X_1X_2Y\bX_1}$.
% \end{corollary}

For any joint type $Q_{X_1X_2Y\bX_1}\in \cP_{\delta}$, we have $d_{TV}(Q_{X_1X_2Y\bX_1},P_{X_1X_2Y}W_{1})\leq \sqrt{\frac{\delta}{2}}$ (using Pinsker's inequality). Setting $\beta = \sqrt{\delta/2}$, we conclude from Corollary~\ref{corollary: 17} that 
\begin{align*}
\gamma''&(\beta, \delta)\geq \bbP\inp{f(X_1, X_2, Y)\neq g(\bX_1, X_2, Y)}\\
&\sum_{x_1,  x_2, y, \bx_1}Q_{X_1X_2Y\bX_1}(x_1, x_2, y, \bx_1)\mathbb{1}_{\inp{f(x_1, x_2, y)\neq g(\bx_1, x_2, y)}}.
\end{align*}
For $\gamma(\delta):=\gamma''(\sqrt{\delta/2}, \delta)$, we conclude that for all sequences $(x_1^n, x_2^n, y^n, \bx_1^n)$ of joint type $Q_{X_1X_2Y\bX_1}$, we have $\ham(f(X_1^n,X_2^n,Y^n),g(\bX_1^n,X_2^n,Y^n)\leq \gamma(\delta)$. Hence, $A = 0$.



% Under $Q_{X_1X_2Y\bX_1}$, we can show that $\sum_{x_1}P_{X_1X_2Y}(x_1, \cdot, \cdot, \cdot)W_{1}\in \cV_1^{\delta+\beta} \cap \cV_2^{\delta+\beta}$. Then, from lemma 4, under $Q_{X_1X_2Y\bX_1}$, we have $\bbP\inp{f(X_1, X_2, Y)\neq g(\bX_1, X_2, Y)}\leq \gamma'(\beta  +\delta)+\beta$. Choose $\gamma''(\beta, \delta) = \gamma'(\beta  +\delta)+\beta$. We choose $\beta = \sqrt{\frac{\delta}{2}}$. Then, $A = 0$.
\fi
\red{*****************************}
